A Conceptual Framework for Refining Influence Knowledge from Simulation Evidence in Cyber-Physical Systems

Cyber-physical systems (CPS) are typically developed by multiple stakeholders who produce artefacts tailored to their specific domains of expertise. The behaviour of these systems emerges from the interaction between those artefacts and their operational environment. Simulation and co-simulation have become essential approaches for analysing CPS behaviour and, through simulation campaigns, developers can explore system responses under changing conditions, including interactions with the environment. However, the lack of details and understanding of some environmentmediated interactions (typically the ones beyond direct sensing and actuation), which remain unmodelled due to their complexity, a lack of time, or a lack of domain experience, hinders the proper comprehension and exploitation of simulation results. To address these limitations, we propose a conceptual framework leveraging the novel concept of Influences to support the iterative and incremental refinement of simulation campaigns and deepen the understanding of the system behaviour. We demonstrate the proposed approach through a case study involving a mobile robot implemented using Simulink/Gazebo co-simulation.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.16   Emergency release: fixes a typo in the code.

Version 2.15   Bug fixes.  Documentation updates
	       New journals: AILET, TAIS, TAISAP, ACMJDS

Version 2.14   Bib style update.  Documentation update.  DLT is now using
	       acmlarge format.
	       Generate error if a user tries to redefine sectioning commands

Version 2.13   Documentation update
	       Added mathcal in unicode mode
	       Bug fixes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/evaluation.tex <==
The campaign is configured from the initial influence model shown in table \ref{tab:influenceUse} and Figure \ref{fig:influencesDiagram}, following the methodology introduced in Section \ref{influence-aware-workflow}. The simulation team together with the domain experts, selects the participants and their baseline values to explore, the SRPs to compute, and the requirement predicates to evaluate from the influence structure itself. %The design artifacts exposed for tuning includes the linear velocity $v_{nominal} \in \{0.3,0.4,0.5\}$ m/s, angular gain $w_{gain} \in \{0.2,0.3,0.4\}$, and the target blob-size threshold $blobsize \in  \{70,120,160\}$ pixels.The environmental factors are $friction_{surface} \in \{low,high\}$ and $luminosity_{level} \in \{low,high\}$. This yields a campaign of $3 \times 3 \times 3 \times 2 \times 2 = 108$ configurations. Table \label{tab:participants-values} summarize the participants and its values.


% \begin{table}[h!]
% \centering
% \caption{Design choices and environmental factors for requirements analysis (SI units).
% We sweep \texttt{$v_{nominal}$} over $\{0.20, 0.30, 0.40\}$\,m/s and
% \texttt{$w_{gain}$} over $\{0.06, 0.07, 0.08\}$, and \texttt{$blob_{size}$} over $\{70,120,160\}$. The \texttt{$friction_{surface}$} sweeps in, the \texttt{$luminosity_{level}$} sweeps between }
% \label{tab:participants-values}
% \begin{tabular}{l l c c}
% \toprule
% \textbf{Category} & \textbf{Participant} & \textbf{Unit} \\
% \midrule
% \multirow{Design Artifacts}
% & \texttt{$v_{nominal}$}  & m/s & $\{0.30, 0.40, 0.50\}$ \\
% & \texttt{$w_{gain}$}& - & $\{0.2, 0.3, 0.4\}$  \\
% & \texttt{$blob_{size}$}& pixels & $\{100,140,180\}$\\
% \midrule
% \multirow{Environmental Factors}
% & \texttt{$friction_{surface}$} & -- & low, high  \\
% & \texttt{$luminosity_{level}$} & -- & low, high \\
% \bottomrule
% \end{tabular}
% \end{table}



\begin{figure*}[h!]
\centering
\includegraphics[width=\linewidth]{images/influencesSignFollow.png}
\caption{KLight Diagram of the initial influences modeled with DemIstifyCPS.}
\label{fig:influencesDiagram}
\end{figure*}



\subsection{Simulation execution}
The co-simulation campaign was executed on an HP EliteBook 840 G10 workstation equipped with a 13th Gen Intel Core i7-1370P processor and 64 GB of RAM, running Ubuntu 22.04.5 LTS. The models and control logic were executed using MATLAB/Simulink (2024a), interfaced via ROS with Gazebo. The Gazebo simulation and TurtleBot3 physical kinematics are hosted within a Virtual Machine.



\subsection{Campaings Compositional Analysis}
\begin{table*}
  \caption{Overview of the methodology sequence for the campaigns, based on the influence model.}
  \label{tab:campaign-overview}
  \small
  \begin{tabular}{p{0.08\textwidth}p{0.14\textwidth}p{0.18\textwidth}p{0.14\textwidth}p{0.17\textwidth}}
    \toprule
    \textbf{Campaign} & \textbf{Block} & \textbf{Inputs} & \textbf{Output} & \textbf{Notes}\\
    \midrule
    P & I\_Perception & AmbientLighting, BlobSize & SignDetectionQuality & Produces bounds for Campaign C\\
    S & I\_Slippery & vNominal, FrictionCoef & AverageSegmentSpeed & Produces SD bounds for Campaign M\\
    C & I\_ControlStability & wGain, SignDetectionQuality & TrackingError & Uses bounds TE from Campaign P\\
    M & I\_MissionPerformance & TrackingError, AverageSegmentSpeed, BlobSize, vNominal & TimeTurning & Uses TE bounds from Campaign C and AS bounds from Campaign S; BlobSize and vNominal use the original design bounds\\
    \bottomrule
  \end{tabular}
\end{table*}


\begin{table*}
  \caption{Campaign-level specification for the modular Morris analysis.}
  \label{tab:campaign-specifications}
  \small
  \begin{tabular}{p{0.06\textwidth}p{0.25\textwidth}p{0.12\textwidth}p{0.20\textwidth}p{0.11\textwidth}p{0.16\textwidth}}
    \toprule
    \textbf{Campaign} & \textbf{Inputs and bounds} & \textbf{Output} & \textbf{Purpose} & \textbf{Run count} & \textbf{Downstream product}\\
    \midrule
    P & AmbientLighting in $[0.3,0.4]$; BlobSize in $[110,130]$ & SignDetectionQuality & Quantify how illumination and apparent target size affect perception quality & $(2+1)\times 10 \times 2=60$ & Derive $SD_{low}$ and $SD_{high}$ from valid aggregated SD values\\
    S & vNominal in $[0.2,0.4]$; FrictionCoef in $[0.4,0.7]$ & AverageSegmentSpeed & Quantify how nominal speed and surface friction affect realized segment speed & $(2+1)\times 10 \times 2=60$ & Derive $AS_{low}$ and $AS_{high}$ from valid aggregated AS values\\
    C & wGain in $[0.2,0.3]$; SignDetectionQuality in $[SD_{low},SD_{high}]$ & TrackingError & Quantify how controller tuning and upstream perception quality affect control stability & $(2+1)\times 10 \times 2=60$ & Derive $TE_{low}$ and $TE_{high}$ from valid aggregated TE values\\
    M & TrackingError in $[TE_{low},TE_{high}]$; AverageSegmentSpeed in $[AS_{low},AS_{high}]$; BlobSize in $[110,130]$; vNominal in $[0.2,0.4]$ & TimeTurning & Quantify how direct mission-level influencers in the graph affect efficiency & $(4+1)\times 10 \times 2=100$ & Final mission-level Morris indices for TimeTurning\\
    \bottomrule
  \end{tabular}
\end{table*}

% \begin{table}
%   \caption{Downstream bound extraction rules for intermediate SRPs outputs.}
%   \label{tab:bound-rules}
%   \small
%   \begin{tabular}{p{0.26\columnwidth}p{0.66\columnwidth}}
%     \toprule
%     \textbf{Variable} & \textbf{Bound Extraction Rules}\\
%     \midrule
%     SignDetectionQuality & $SD_{low}=\max(0,P5(SD))$, $SD_{high}=\min(1,P95(SDQ))$\\
%     AverageSegmentSpeed & $AS_{low}=\max(0,P5(AS))$, $AS_{high}=P95(AS)$\\
%     TrackingError & $TE_{low}=\max(0,P5(TE))$, $TE_{high}=P95(TE)$\\
% %    Fallback rule & If the sample is small and clean, raw minimum and maximum values may be used for a deliberate wider stress-test analysis\\
%     \bottomrule
%   \end{tabular}
% \end{table}


\begin{table}[t]
\caption{Quantile-based operating regimes used for intermediate SRPs.}
\label{tab:srp_regimes}
\centering
\begin{tabular}{ll}
\toprule
\textbf{Regime} & \textbf{Quantile interval} \\
\midrule
Low       & $[P_{0}, P_{25}]$ \\
Moderate  & $(P_{25}, P_{50}]$ \\
High      & $(P_{50}, P_{75}]$ \\
Very High & $(P_{75}, P_{100}]$ \\
\bottomrule
\end{tabular}
\end{table}
\subsection{Results}
We perform an individual participant analysis, in which one participant is varied and the resulting effect on the SRPs are observed. In a second step, we perform a combined analysis within each influence, in which the participants of the same influence are considered jointly, to observe if the influence of one participant changes because of the change of another one, as a cross-integration effect . In a third step, we quality the observed effects as beneficial or prejudicial, and the existence of trade-offs with respect to the SRPs and requirements. 

\subsubsection{Step1: Individual influence}
For each participant, we compute three descriptive indicators. The SRP range, as the difference between the smallest and the largest SRP value observed with the tested values. The second is the mean stepwise SRP change, as the average magnitude change between the consecutive participant's values. These indicators provide an initial measure of how strongly variations in a participant are reflected in the variation of an SRP.


Figure \ref{fig:vnominal} shows the results of varying $v_{nominal} $ with respect to the SRP \texttt{AverageSegmentSpeed}. In Table \ref{tab:vnominal}, we summarize how the change of the participant reflects in the variation of the SRPs. The results shows that $v_{nominal} $ has the strongest effect on \texttt{AverageTravelSpeed(old influence)} of 46.64\%, followed by \texttt{TrackingErrorRMS} and \texttt{AverageSegmentSpeed} around 33\%. Its effect on \texttt{SignDetectionQuality} is weaker, with a relative range of 12.35\%. This suggests that nominal speed acts primarily on motion and performance-related SRPs, with a small propagated effect on perception quality.

% \begin{table*}[h!]
% \centering
% \caption{Indicators for the participant $v_{nominal} \in \{0.25, 0.35, 0.45, 0.55\}$ m/s.  The other participants are fixed, with $luminosity_{level}= high$, $friction = low$, $w_{gain} = 0.25$}
% \label{tab:vnominal}
% \begin{tabular}{lllllll}
% \hline
% \textbf{SRP} & \textbf{Min} & \textbf{Max} & \textbf{Range} & \textbf{Mean step change} & \textbf{Relative range (\%)} & \textbf{SRP impact} \\
% \hline
% AverageSegmentSpeed    & 0.225   & 0.302   & 0.077  & 0.026  & 29.32 & beneficial             \\
% SignDetectionQuality   & 0.856   & 0.914   & 0.058  & -0.016 & 6.58  & mixed, net prejudicial \\
% TrackingErrorRMS       & 134.684 & 194.006 & 59.322 & 16.656 & 36.14 & mixed, net prejudicial \\
% AverageTravelSpeed     & 0.085   & 0.151   & 0.066  & -0.015 & 51.11 & mixed, net prejudicial \\
% TimeTurning   & 10.060  & 16.867  & 6.807  & 1.256  & 50.90 & mixed, net prejudicial \\
% \hline
% \end{tabular}
% \end{table*}



In Table \ref{tab:wgain}, we summarize how the change of the participant reflects in the variation of the SRPs. The results shows that $w_{gain} $ has a strong effect on \texttt{TrackingErrorRMS}, followed by \texttt{AverageTravelSpeed}. The effects on the \texttt{AverageSegmentSpeed} and \texttt{SignDetectionQuality} are weak, which shows that this participant have stronger influence in control SRPs, not being so influential on the perception quality. 


% \begin{table*}[t]
% \centering
% \caption{Indicators for the participant $w_{gain} \in \{0.15, 0.25,0.35,0.45\}$. The other participants are fixed, with $luminosity_level= high$, $friction = low$, $w_{gain} = 0.25$, $v_{nominal} = 0.25$ }
% \label{tab:wgain}
% \begin{tabular}{lllllll}
% \hline
% \textbf{SRP} & \textbf{Min} & \textbf{Max} & \textbf{Range} & \textbf{Mean step change} & \textbf{Relative range (\%)} & \textbf{SRP impact}  \\
% \hline
% AverageSegmentSpeed  & 0.224 & 0.227 & 0.004 & 0.002 & 1.65 & beneficial\\
% SignDetectionQuality & 0.903 & 0.940 & 0.036 & 0.015 & 3.92 & beneficial \\
% TrackingErrorRMS     & 118.747 & 139.098 & 20.351 & - 6.784 & 15.93 & beneficial\\
% TimeTurning & 8.340 & 10.340 & 2.000 & - 0.667 & 21.04 & beneficial \\
% \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[t]
% \centering
% \caption{Indicators for the participant $target\_blob\_size \in \{\}$. The other participants are fixed, with $luminosity_level= high$, $friction = low$, $w_{gain} = 0.25$, $v_{nominal} = 0.25$ }
% \label{tab:wgain_blobsize}
% \begin{tabular}{lllllll}
% \hline
% \textbf{SRP} & \textbf{Min} & \textbf{Max} & \textbf{Range} & \textbf{Mean step change} & \textbf{Relative range (\%)} & \textbf{SRP impact} \\
% \hline
% AverageSegmentSpeed    & 0.207   & 0.228   & 0.022  & 0.007   & 9.81  & beneficial            \\
% SignDetectionQuality   & 0.828   & 0.931   & 0.104  & 0.024   & 11.64 & mixed, net beneficial \\
% TrackingErrorRMS       & 133.537 & 166.026 & 32.489 & -10.002 & 22.71 & mixed, net beneficial \\
% AverageTravelSpeed     & 0.087   & 0.130   & 0.043  & 0.014   & 37.19 & beneficial            \\
% TimeTurning   & 11.260  & 18.875  & 7.615  & -2.258  & 56.85 & mixed, net beneficial \\
% \hline
% \end{tabular}
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{Indicators for the participant $luminosity\_level \in \{\}$. The other participants are fixed, with $target\_blob\_size = 120$, $friction = low$, $w_{gain} = 0.25$, $v_{nominal} = 0.25$ }
% \label{tab:luminosity}
% \begin{tabular}{lllllll}
% \hline
% \textbf{SRP} & \textbf{Min} & \textbf{Max} & \textbf{Range} & \textbf{Mean step change} & \textbf{Relative range (\%)} & \textbf{SRP impact} \\
% \hline
% AverageSegmentSpeed    & 0.220   & 0.227   & 0.007 & -0.001 & 3.24  & mixed, net prejudicial \\
% SignDetectionQuality   & 0.892   & 0.915   & 0.023 & 0.005  & 2.50  & mixed, net beneficial  \\
% TrackingErrorRMS       & 138.942 & 140.644 & 1.702 & 0.169  & 1.22  & prejudicial            \\
% AverageTravelSpeed     & 0.124   & 0.140   & 0.015 & -0.004 & 11.73 & mixed, net prejudicial \\
% TimeTurning   & 9.033   & 12.380  & 3.347 & 0.730  & 31.05 & mixed, net prejudicial \\
% \hline
% \end{tabular}
% \end{table*}


\subsubsection{Step2: Check Interaction Changes individual influence?}
Three graphs SRP average speed vs friction vs vnominal
Three graphs SRP quality vs luminosity vs blobSize

These results shows how the participant's effect changes according to the variation of other participants.
\subsubsection{Step3: Beneficial/prejudicial}

\subsection{Divide and Conquer Composition of Influences}
Influence ControlStability has inputs of SignDetectionQuality and AverageSegmentSpeed. Those SRPs interact with wgain, and produce the srp tracking error. To analyse the effects of the srps on the influence, we have chosen 3 regimes for each of them, in which we consider for the campaign.

Performing compositional analysis, helps understanding better each of the couplings, providing a better undersatnding of the interactions between the participants of each influence.


Campaign P answers the questions:
Does lighting matter more than blob size for perception quality?
Is the effect nonlinear or interaction-heavy?
Campaign S answers:
Is average segment speed more sensitive to nominal speed or friction?
Does friction create strong nonlinear behavior?
Campaign C answers: Is tracking error driven more by controller tuning or by degraded perception quality?
Does poor perception amplify control instability?

==> sections/influence-aware-worflow.tex <==
This section positions Influence modeling and simulation within the CPS lifecycle and clarifies how it can be exploited at design time. %We explain how we understand Influences can be obtained, and managed by stakeholders. 
We present how the Influence modeling and static analysis provide early feedback during the design phase. %, providing insights for developers for choices in system models. 
The other part, we show how we plan to use simulation outcomes to refine influence knowledge, especially when influence functions are not yet available.

Figure \ref{fig:workflow-implementation} summarizes the proposed influence-aware modeling and simulation and its exploitation for development activities. %, across design and simulation.

\begin{figure*}[h!]
\centering
\includegraphics[width=0.8\linewidth]{images/workflow.png}
\caption{CPS Influence Workflow with Influence modeling and analysis across design, and simulation phases.}
\label{fig:workflow-implementation}
\end{figure*}


As shown in the figure, the first stage is the \textbf{(1) Design System Models and Influence Model}, when stakeholders specify requirements, developers of each domain define their initial system design artifacts. For example, they may define SysML, Capella, AADL.
Following that, the same developers, or specialized ones (e.g. system integration engineer), use those artifacts as references to identify and document Influences. The level of detailing is flexible, as the developers are able to document according to different levels of abstraction, ranging from the use of informal rationales to quantitative functions. They can partially express the influences according to their experience and understanding of system behavior. %They can define what artifacts and cyber physical phenomena they have already identified to be participants of influences, what are the requirements that may be dissatisfied. 

%Ok, but later, iteration Additionally, they can detail what are the confidence levels on the definition of the influences. Moreover, if they had already gathered information of the system behavior in runtime, they can add metadata of likelihood and other metrics to evaluate the influence impacts.

%During the initial iterations of CPS development, it is unavoidable that developers do not have fully understanding and documented information needed for the Influence Modeling. They can partially express the influences according to their experience and understanding of system behavior. %The influences not yet discovered or partially understood may be clarified and added to the Model in the other phases of the development process.

%The still uncovered influences can be discovered and added to the model after the first design phase, as an iteration with knowledge discovered during system operation. 

In step \textbf{(2) Analyze Influences}, the Influence Model is transformed into graphs and analyzed structurally and, if possible, quantitatively. It aims at analysing the system without simulating or operating the CPS, solely by analyzing statically the models defined at design time. 
As results of the static analysis, we compute indicators such as: (i) impact rankings for influence participants, (ii) reachability of participants, (iii) if influence functions are numeric, determine whether participants are \emph{beneficial} or \emph{prejudicial} to requirement satisfaction, ranking them by feasibility or changeability when metadata is available.

In step \textbf{(3) Generate Analysis and Compensation Suggestions}, the tool provides the results of the analysis to developers. Actionable suggestions are presented in the host modeling tools, e.g. SysML models, raising info, warning markers and live edit messages. %that inform how the current change in a participant is expected to affect a specific system response property and related requirements. 
In this way, developers can inspect propagation paths, the criticality of their changes and make informed decisions. The designers can proceed with iterations on the models, adjusting, and validating system design.

%The evaluation of requirement satisfaction are be provided as a binary result, if the system requirement is satisfied or not, or as a satisfaction degree score, evaluating from [0,1] the satisfaction of results.



%With that, the impact of the influences are evaluated, and feedback is provided to the users accordingly.  With that, we can understand the relevance of system influences.
During the initial iterations of CPS development, it is unavoidable that developers do not have fully understanding of system influences. As a result, the feedback after analysis can be limited. To complement this early analysis, we introduce the use of simulation for improving the understanding of system behavior and the refinement of the influences.

The lower part of the diagram shows \textbf{Influence-Guided Simulation}.% Engineers proceed with exploration of the initial influence models.
In \textbf{Step (4): Configure the Simulation Campaign} simulation engineers configure the simulation runs aligned with the influence models. %This involves selecting the artifacts or environmental factors expressed as participants in Influence model, to observe how the system behaves in runtime, according to relevant ranges of the same parameter or environment factor. 
The simulation's goal is not focused on validation of behavior or optimization of design. It serves to reveal whether and how specific design artifacts choices and environmental factors are affecting system behavior. %, and possibly dissatisfying requirements.

With the simulation logs and traces, the workflow proceeds to \textbf{Step (5): Capture and Structure Evidence}. We propose the enrichment of the influence models according to simulation evidence %, possibly providing influence analyzable functions. Following that, with the enriched model, the tool can analyze influences and computes quantitative requirement satisfaction. 
Feedback is provided to domain experts, together with recommendations of refinement on the influence definition. %The personalized feedback to the concerned developers improves the collaboration and accelerates the reasoning on decisions to maintain system requirements satisfaction.

In the next section, we propose a detailed methodology for influence-guided simulation, that we will demonstrate in this paper with the motivating use case.

%Influence Model can be updated based on these observed outcomes, and developers can iterate on the existing  definition of influences and possibly discover new ones, and to identify new possible violations of requirements which could not be identified during static analysis. 
%The requirement violations are further evaluated for the selection of target design choices that can be modified to restore the requirement satisfaction. 
%We recommend design choices on target artifacts to the users that restore and improve the satisfaction of requirements.



% Such influences arises naturally from the combination of design choice on the source artifact and the surrounding phenomena. For example, it includes the time to stop the robot's movement, how the battery state of health under specific phenomena and choices on source artifacts.
% The computation may involve using physical laws, mathematical equations and logic rules, combining the observed effects of the inputs as a explicit formulation. 
% The relation between parameters of the design artifacts and the cyber physical phenomena can be expressed in different levels of abstraction, by physical laws,y = f(x1,x2,x3), or more informal definitions, "when the wind is strong, and i have chosen a high speed".






% \section{\textcolor{red}{Evaluation}, actually Discussion? : Influence Concept Coverage}
% \label{sec:discussion}
% Our goal is to discuss to what extend of the Influence concept covers the implicit relations within system and environment. 
% We discuss our proposal based on the coverage of the requirements we have set in Section \ref{subsec:requirements} and the effectiveness of the usage of the tooling on the use case we have developed, as depicted in Section \ref{sec:motivation}.
% The tooling is used as evidence of how the concept can be operalized in CPS development, demonstrates how modelers can interact with it, and supports typical design and verification activities on the use case.
% The use case is an evidence of practicality.

% \subsection{Coverage of Influence Concept}
% \subsubsection{According to RQ1: Explicity modeling} The definition of an influence turns implicit relationships into explicit modeling, with well defined roles: originators (artifacts, phenomena), a system response (what is the system behavior at runtime), and a rationale, that explains their interplay. By making these roles explicit, the model provides clarity of how the design changes in artifacts and environmental factors jointly shape system response.


% For example, in the Cherokey use case, the design artifacts such as motor speed, motor type, and the phenomena such as surface friction and slope are linked thought the concept of influence, which is specified with a rationale how they affect stopping distance. The rationale describing the influence specifies the reasoning of this relation, making the relation explicit in the model rather than implied. This enables stakeholders to interpret the system responses more effectively than if they remain hidden or only discovered when the system is in runtime.


% \subsubsection{According to RQ2: System Operational Context}
% The Influence concept captures the how the environmental phenomena and design artifacts interact under specific contexts, without the need of full physics-level modeling. Influences clarify when and where they are pertinent, by the assumptions, boundaries or mathematical expressions when available.

% For example, in the Cherokey use case, an influence can record the observed condition: when the motor speed exceeds 20 cm/s and the slope is greater than 30 $^{\circ}$ , the displacement surpasses the 5 cm threshold required by RQ2 (Obstacle Avoidance). This is an alternative of encoding the full kinematic equations, which could be unnecessary and time consuming.

% \subsubsection{According to RQ3: Requirement traceability}
% The concept covers end-to-end traceability, linking design choices and phenomena to system responses and, in turn, to requirements. This allows to reason not only whether requirements are satisfied, but also how design changes in artifacts propagate through the system. By explicitly representing these links, the model provides explainability of requirement satisfaction, developers can see why a requirement is not validated, trace back to the specific design artifacts or phenomena that contributed to the outcomes, allow the calculation of candidates for compensation.

% For example, starting from the requirement \texttt{obstacleAvoidance}, the model explicit the chain:
% $\texttt{obstacleAvoidance} \rightarrow \texttt{DistanceCalculationAccuracy} \rightarrow \texttt{Influence5}$,
% and $\texttt{Influence5}$ is driven by \texttt{sweepDelay} together with the \texttt{wavePropagation} system response.
%  The same path works forward: for the artifact \texttt{sweepDelay}, the concept immediately provide the information of which system responses it may affect and the related requirements. 
%  This is a direct result from the explicit roles defined in the Influence concept and the semantics attached to them.

% \subsubsection{According to RQ4: Support interactions and propagation effects}
% The Influence concept goes beyond capturing direct relations between artifacts and phenomena. It supports reasoning about interactions that propagate across the system, where the linked system responses from influences can be originators of other influences, ultimately affecting a requirement satisfaction.

% In the use case, the ultrasonic sensor and environmental phenomena influences the \texttt{wavePropagation} response. This response, combined with the artifact \texttt{sweepDelay}, generates a new system response describing motion of the sensor during measurement. In its turn, this response participates as an originator in another influence, affecting the requirement RQ2 Obstacle Avoidance. This helps understanding more complex aspects of influences, such indirect requirement violations, and trade-offs between artifacts of different influences.


% \subsection{Example of tooling usage}
% We have instantiated the Influence Model with the use case of Cherokey 4WD mobile robot (Sec.~\ref{sec:motivation}), modeled in SysML v2.

% In the Cherokey model, influences refer directly to existing SysML~v2 elements such as \texttt{activityDynamicDetection.detectionThreshold}, \texttt{activityDynamicDetection.sweepDelay}, and \texttt{Cherokey4WDModel.PartDefinitions.Battery}, as well as phenomena including \texttt{temperature} and \texttt{surfaceFriction}. System responses are explicit, named predicates, such as \texttt{TravelSpeedInOperation}, \texttt{TimeToCompletelyStop}, which appear in the model as first-class objects and can be reused across influences and requirements.

% An important aspect of our contribution is that domain specific models do not need to be modified. Instead, the formalism of Influence allows the usage of objects from their models. When the objects are changed in their nominal model, the Influence tooling monitors these modifications and generates feedback. The warnings and flags are not only isolated in the Influence Model, but are displayed in the developer's models directly. 

% This integration demonstrates the practicality of the Influence concept and tooling. Domain experts can continue working on their familiar and standard models and tools, and Influence acts as another layer or cross-cutting construct.
% This ensures that guidance is provided when and where exactly the model edits actually occurs, improving explainability and coordination without intruding on standard modeling practices.


% % What we monitor?

% % The framework is restrictive. 

% % The output of an influence was an artifact, now is not anymore.


% \subsection{Practical Applicability and Open Challenges of our Proposal}
% We have demonstrated clear benefits of our proposal for CPS development. This section discusses the scope on its applicability and open challenges we have identified.

% One of the challenges of this work is the exploration of the CPS development has been conducted on a single use case, the Cherokey 4WD robot. Although it is a small use case, the study demonstrated that the approach is beneficial even when applied to small usage, with limited numbers artifacts. Therefore, there is a need for broader validation, exploring larger uses cases, and to realize a further evaluation involving multiple teams and organizations. Moreover, there is a need to demonstrate the tooling with different MBSE practices and toolchains, so that the concept can be validated across different toolings and modeling environments.



==> sections/introduction.tex <==


Cyber-physical systems (CPS) are developed by multiple stakeholders who create artefacts according to domain-specific concerns. This makes CPS development a socio-technical activity, where system integration depends on the coordination of decisions across heterogeneous artefacts \cite{carreira2020multi,combemale2014globalizing}.

A challenge in CPS development is that system behaviour is not just the sum of isolated components.  Instead, CPS behaviour emerges from couplings \textit{within} the System Under Study (SUS) and \textit{between} the SUS and the environment where the CPS operates~\cite{lee2008cyber}. While some couplings arising directly from sensing and actuation are well understood, others remain unmodeled due to complexity, a lack of time or a lack of domain experience. In particular, environment-mediated interactions are often overlooked despite their critical role in shaping system outcomes. To address this, recent work has introduced the notion of \textit{influences}, which capture how design artefacts and environmental factors jointly affect System Response Properties (SRPs) -- \ie, observable system outcomes such as braking distance or tracking error that ultimately determine requirement satisfaction \cite{da2026demistifycps}. Influence modelling is related to dependency and causal modelling approaches, but differs in its explicit representation of environment-mediated interactions and their impact on system-level properties.
The specification of an influence can take various forms, ranging from natural language to formal mathematical functions, depending on stakeholder knowledge. While qualitative analysis is possible with natural language descriptions -- typically to provide insights about the impact of modifying artefacts or environmental factors --, mathematical functions enable quantitative analysis and recommendation algorithms for socio-technical coordination -- typically to determine whether changes to design artefacts or environmental factors have a positive or negative impact on requirement satisfaction and to rank design alternatives based on their expected impact on requirement satisfaction.
%
However, in early development, influence models are usually not fully defined. Engineers often have partial or intuitive knowledge about relevant factors but lack precise models of their interactions. Consequently, influence models remain incomplete, limiting their analytical usefulness and preventing their effective use in guiding design decisions. In current CPS practices, simulation is used to gain knowledge about the system and its potential influences. However, simulations typically generate large volumes of data without systematically structuring the resulting information or feeding this information back into system models to improve their structure or completeness. 

To address this limitation, we propose a closed-loop approach for the systematic structural and functional refinement of influence models using simulation evidence. In our approach, influence models play a dual role. First, they act as a guide by identifying relevant artefacts, environmental factors, and SRPs, thereby structuring and constraining simulation campaigns. Second, they serve as an actionable modelling artifact for knowledge, where evidence extracted from simulation traces is used to refine, extend, and revise influence relationships.

Building on the DemIstifyCPS framework, our approach enables the systematic refinement of influence definitions into forms amenable to quantitative analysis and supports the identification of structural gaps by uncovering previously unknown design artefacts or environmental factors affecting specific SRPs. In this way, simulation is not only used for validation but also as a means to incrementally construct and improve influence models, \ie, system knowledge.

The main contributions of this paper are as follows:
\begin{itemize}
\item \textbf{An influence-guided simulation methodology:} A framework that leverages influence models to design and structure simulation campaigns, extract System Response Properties from execution traces, and align simulation evidence with model elements.
\item \textbf{Simulation-driven refinement of influence models:} a method to systematically update and extend influence relationships based on simulation data, improving model completeness. %enabling the discovery of previously unmodeled factors and improving model completeness.
\end{itemize}

We demonstrate the proposed approach through a case study involving a mobile robot implemented using Simulink/Gazebo co-simulation. The results show that structuring simulation evidence through influence models improves the understanding of system behaviour and supports more informed design decisions.

The remainder of the paper is organized as follows. Section \ref{related} presents the foundations and related work of this paper. Section \ref{influence} presents the concept of Influence and the DemIstifyCPS DSL. Section \ref{motivating-example} introduces the running example that we use in the paper. Section \ref{influence-aware-framework} discusses how the Influence Modelling is exploited across development activities. Section \ref{methodology} presents the conceptual framework for influence-guided simulation and model refinement. Section \ref{evaluation} presents the evaluation results. Section \ref{discussion} discusses the perspectives and the limitations of this work. Section \ref{conclusion} concludes the paper and presents future work.

==> sections/methodology.tex <==
This section presents a methodology for conducting simulation campaigns guided by an influence model and to exploit the simulation traces to better understand SRPs and to refine influence model.

To apply the methodology, we rely on a tool chain including DemIstifyCPS DSL for influence modelling, MATLAB/Simulink and Gazebo for simulation implementation, and Python notebooks for analysis of simulation outcomes.
Influence knowledge is first modelled in the DemIstifyCPS DSL, and domain models are managed in their respective system-models environments. The simulation campaign is performed with a co-simulation toolchain: MATLAB/Simulink implements the control and decision logic, ROS handles communication, and Gazebo simulates the physics, with Gazebo Pacer handling the synchronization across the simulation components. The runs produce traces, logged signals, that are used to compute SRPs. Finally, with the use of Python notebook, analysis produces plots, summary statistics, proposal of influence functions. These analyses are provided to domain experts so they understand better system behaviour and realize further refinement in the influence model. Figure \ref{fig:workflow-implementation} represents the process, that will be detailed in the following subsections. %After domain experts had defined their influences,  %and the simulation workflow follows the partial modeled knowledge of the influences. Based on this model, 
%engineers configure the simulation runs from this initial influence model. The simulation logs are related to SRPs and requirement margins that can be compared across runs.

\begin{figure*}[h!]
\centering
\includegraphics[width=0.9\linewidth]{images/sim_campaigns.png}
\caption{Methodology for Simulation Campaigns with the guidance of the Influence Model.}
\label{fig:workflow-implementation}
\end{figure*}


\subsection{Inputs and configuration of simulation campaign from the influence model}


The simulation campaigns are configured from the initial influence model, which may be incomplete. From each influence, the model identifies design artifacts, environmental factors, input SRPs and outputs SRPs to be explained. This structure is used to define the simulation campaign. In this way, instead of exploring the possible large parameter space of the simulation without a defined strategy, the campaign focus on the participants that are linked to the SRPs under study. This keeps the exploration consistent with the knowledge from the influence models.
%\subsubsection{Environmental factors and artifacts definition}

%In this model, environmental factors are treated as first-class modeling construct with the artifacts, and both appear as participants in an influence. Each participant is related to simulation parameters, with a baseline numeric value for exploration (e.g. \texttt{$v_{nominal}$} m/s in $\{0.30, 0.40, 0.50\})$. %or an admissible range or discrete levels. 
%These numeric values are defined by the developers, that  from the system models made reference in the influence model, and environmental factors settings defined in it.

The campaign specification defines the map to the simulation parameters, with a range for exploration. Depending on the type of parameter, this can be defined as a category condition (e.g. high or low \texttt{luminosity}) or a baseline numeric value (e.g. \texttt{$v_{nominal}$} m/s in $\{0.30, 0.40, 0.50\})$. %\subsubsection{System-Response Properties}
Each run is assigned metadata to support reproducibility and traceability. This metadata includes a campaign identifier and participants identifier and settings, and a random seed (including randomized run ordering). To ensure comparability between runs, the campaign defines the number of replicates per configuration, 
%to separate systematic effects from noise or nondeterminism. It also defines the number of replicates per configuration
timeouts and final events (e.g., task completed, collision detected, etc), invalid run conditions (e.g., missing signals, synchronization failure).
%\subsubsection{Requirement}



% SRPs are extracted or computed from logs and raw traces of the simulation. Typical examples include signal detection rate, tracking error magnitude, collision count, minimum distance margin, or control effort measures.
% Requirements are evaluated from SRPs numeric values. A requirement can be represented as a margin that quantifies how far the observed behavior is from the satisfaction or violation boundary, or as a boolean predicate, indicating whether a run satisfies or violates the requirement.


\subsection{Simulation execution and trace collection}
Once the campaign is specified, the simulation executes two run for each configuration. This methodology assumes an orchestration mechanism capable of synchronization between simulators, including time-step coordination and data exchange policies to ensure that traces are interpretable and comparable across runs. 

The logging configuration is derived from the SRPs that need to be evaluated. It includes outputs (e.g., position, velocity, mode/state-machine state), control commands, perception outputs (e.g., detection confidence, tracking error), discrete events (e.g., stop triggered, contact/collision event, mode transition), timing signals (e.g., timestamps, step counters). %The logging configuration is aligned with the influence model, and some of the logs are chosen so they support SRP computation.
%Each run produces a record that includes: configuration, with particpants ID, participant settings, raw logs/traces (time series, events), derived results, SRPs and requirement margins and outcomes of requirement evaluation.

\subsection{SRP extraction and Requirement Evaluation}

The raw traces are transformed into SRPs. An SRP captures one relevant aspect of system behaviour and can be used either as an input of an influence relation or to be evaluated against a requirement. In this methodology, SRPs are obtained with deterministic functions to traces and discrete events. SRPs can be event-based, derived from the occurrence of specific events (e.g., stop events, collisions), temporal aspects of behaviour (e.g., completion time, detection latency), performance SPRs (e.g., speed average, detection counts).

After multiple runs are collected, the tool chain aggregates run records into summary tables in CSV format with participants ID, participant settings, SRPs values. 
This set of results will be used to refine influence knowledge. It is not only a collection of simulation traces, but a structured evidence that is then exploited for the refinement of influence model and to use for follow-up runs or compensation strategies.

% \begin{table}[t]
% \centering
% \caption{Representative SRPs and log computation used for requirement assessment and explainability.}
% \label{tab:srps}
% \begin{tabular}{p{0.28\linewidth} p{0.66\linewidth}}
% \hline
% \textbf{SRP} & \textbf{Computed from logs} \\
% \hline
% % \texttt{CompletionFlag} &
% % $\texttt{stopRobot}(t)=\texttt{true}$ \\
% % \texttt{CompletionTime} &
% % time for finishing the task and find the sign to stop\\
% \texttt{SignDetectionRate} &
% $\min\{t \mid \texttt{sign}(t)=\texttt{true}\}$ from the moment the robot detects a possible sign to determine that is true \\
% \texttt{TrackingStability} &
% $error(|\texttt{blobX}(t)-x_{\text{center}}|)$ over intervals with \texttt{detected=true}, how far  is from the center of the robot \\
% \texttt{TravelSpeed} &
% $|v(t)|$ (command or odometry) \\
% \hline
% \end{tabular}
% \end{table}

%With each parameter set, it is possible to observe the effect on system behavior according to the specific participants.

Requirement satisfaction is then assessed in a separate step. This allows the same computed SRPs to be reused if the requirements, thresholds, or satisfaction criteria evolve over time. Requirement is evaluated for the SRP summaries, as Boolean predicates, as for the completion flag and completion time, or as requirement margins, as for tracking error magnitude, indicating how close the run is to satisfaction or violation.

\subsection{Analysis and Knowledge Refinement }

The final stage analyses the simulation results to reveal trends and strengthen the semantics of influence relations. As a first part, the analysis is descriptive, to identify overall tendencies. It generates plots and summary statistics to visualize how SRPs varies according to different participant's configurations.
Developers can then identify tendencies of which participant changes affect a given SRP, and which combinations of settings may represent trade-offs on decision-making. For example, the increase of a parameter may decrease the time to complete a task, but at the same time, increase a performance error indicator.

The tool chain provide analysis to understand the effect of one participant on an SRP while keeping the other factors fixed, with a specific chosen scenario. This allows the understanding of the local effect of that participant. Moreover, it provides the analysis of the joint effect of the participants on the SRPs. This is essential for understanding the influences, as the SRP emerges from the interaction of multiple participants, not isolated effects.
%This supports also the identification of most influential participants, verifying what is the effect on the SRP when a particular participant vary.  




% After the runs are executed, the traces are post-processed to compute SRPs. In this use case, the extracted SRPs include travel time, detection rate, and tracking error magnitude, which are computed either directly from logged signals or derived from logs. 




Moreover, when there is enough evidence and the influence relation is empirically supported, a quantitative influence function is derived. In this context, confirming an influence means that the analysed participants show a consistent effect on the target SRP. If the results do not show a tendency, it indicates that the proposed participants may not fully explain the SRP, that other relevant participants are missing, or that the influence is not well formulated or not in an adequate level of abstraction. Influence functions enable quantitative reasoning by providing an explicit mapping from a set of participants (design artifacts and environmental factors) to a single System Response Property (SRP). The resulting function can be incorporated into the influence model as a formalized refinement, together with its validity conditions.

%Each influence function is learned for a single output SRP. With an influence structure, a set of participants is restricted to those structurally connected to the SRP within the influence model. This narrows the design exploration and preserves the alignment between the learned relation and the initial knowledge captured in the model.

%Reasoning on the simulation results can rely on statistical and machine-learning techniques, depending on the data characteristics and the desired level of the interpretation.

==> sections/usecase.tex <==
We demonstrate the proposed workflow on the sign-following robot introduced in Section \ref{motivating-example}. We present the use case through the roles of the domain experts Alice, Bob and Charlie. During development, they define their domain models, and agree on the interfaces between their system parts. As we motivated in the problem definition in subsection \ref{motivating-example-problem}, they realize that changes in artifacts and environmental conditions jointly shape system response properties, and that a systematic workflow is needed to transfer this behavioral knowledge from simulation into the influence model. 

At the beginning of the simulation phase, the three developers already have an initial influence model, with its participants and output SRP depicted in table \ref{influenceUse}, and in Figure \ref{fig:influencesDiagram}. Note that this is a simplified version as there are other participants that may be included in the model. This model does not yet provide complete quantitative functions, but it identifies the main participants, the SRPs of interest, and the requirements they may affect. The purpose of the simulation campaign is to improve understanding of how these participants shape SRPs and requirement satisfaction.
\begin{table}[h!]
\centering
\caption{Influences identified in the use case.}
\label{tab:influenceUse}
\begin{tabular}{p{1.2cm} p{2.5cm} p{2.5cm}}
\toprule
\textbf{Influence} & \textbf{Participants} & \textbf{Output SRP} \\
\midrule
$I_1$ & \texttt{vNominal}, \texttt{wGain}, \texttt{frictionCoef} & \texttt{TravelTime} \\
$I_2$ & \texttt{blobSize}, \texttt{RobotMovement} & \texttt{DistanceToSign} \\
$I_3$ & \texttt{vNominal}, \texttt{wGain}, \texttt{frictionCoef} & \texttt{RobotMovement} \\
$I_4$ & \texttt{luminosity}, \texttt{blobSize}, \texttt{RobotMovement} & \texttt{QualityPerception} \\
\bottomrule
\end{tabular}
\end{table}

\begin{figure*}[h!]
\centering
\includegraphics[width=\linewidth]{images/influencesSignFollow.png}
\caption{KLight Diagram of the initial influences modeled with DemIstifyCPS.}
\label{fig:influencesDiagram}
\end{figure*}


\subsection{Campaign setup}
The campaign is configured from the initial influence model shown in table \ref{tab:influenceUse} and Figure \ref{fig:influencesDiagram}, following the methodology introduced in Section \ref{influence-aware-workflow}. The simulation team together with the domain experts, selects the participants and their baseline values to explore, the SRPs to compute, and the requirement predicates to evaluate from the influence structure itself. The design artifacts exposed for tuning includes the linear velocity $v_{nominal} \in \{0.3,0.4,0.5\}$ m/s, angular gain $w_{gain} \in \{0.2,0.3,0.4\}$, and the target blob-size threshold $blobsize \in  \{70,120,160\}$ pixels.The environmental factors are $friction_{surface} \in \{low,high\}$ and $luminosity_{level} \in \{low,high\}$. This yields a campaign of $3 \times 3 \times 3 \times 2 \times 2 = 108$ configurations. Table \label{tab:participants-values} summarize the participants and its values.


\begin{table}[h!]
\centering
\caption{Design choices and environmental factors for requirements analysis (SI units).
We sweep \texttt{$v_{nominal}$} over $\{0.20, 0.30, 0.40\}$\,m/s and
\texttt{$w_{gain}$} over $\{0.06, 0.07, 0.08\}$, and \texttt{$blob_{size}$} over $\{70,120,160\}$. The \texttt{$friction_{surface}$} sweeps in, the \texttt{$luminosity_{level}$} sweeps between }
\label{tab:participants-values}
\begin{tabular}{l l c c}
\toprule
\textbf{Category} & \textbf{Participant} & \textbf{Unit} \\
\midrule
\multirow{Design Artifacts}
& \texttt{$v_{nominal}$}  & m/s & $\{0.30, 0.40, 0.50\}$ \\
& \texttt{$w_{gain}$}& - & $\{0.2, 0.3, 0.4\}$  \\
& \texttt{$blob_{size}$}& pixels & $\{100,140,180\}$\\
\midrule
\multirow{Environmental Factors}
& \texttt{$friction_{surface}$} & -- & low, high  \\
& \texttt{$luminosity_{level}$} & -- & low, high \\
\bottomrule
\end{tabular}
\end{table}

%These parameters are selected because they are plausible participants in the couplings that affect the SRPs related to the two requirements. 
%The simulation campaign varies these parameters across selected ranges, while keeping track of the scenario, the run ID, and the configuration metadata for each execution.
For each run, the campaign collects the participant settings, the campaign identifier, scenario identifier, run identifier, and execution metadata. The analysis uses \texttt{completion\_time}, \texttt{v\_mean}, \texttt{track\_err\_rms}, and the stopping distances ($d_i$), together with the requirement indicators \texttt{RQ1\_Complete}, \texttt{RQ2\_TravelSpeed}, \texttt{RQ3\_SafeDistance}, and \texttt{RQ4\_Perception}. Table \ref{tab:requirementEv} presents how each requirement is evaluated. The purpose of the campaign is not optimization of the design space, but the refinement of influence to support requirement reasoning.

\begin{table*}[t]
\centering
\caption{Requirement evaluation metrics used in the simulation campaign.}
\label{tab:req-margin-definitions}
\begin{tabular}{p{1.5cm} p{5.0cm} p{7.5cm}}
\toprule
\textbf{Req.} & \textbf{Intent} & \textbf{Evaluation} \\
\midrule

RQ1 &
Complete the task within 60\,s &
$\texttt{RQ1\_Complete}=1$ iff $\texttt{completed}=1 \land \texttt{completion\_time} \leq 60$ \\

RQ2 &
Maintain safe travel speeds &
$\texttt{RQ2\_TravelSpeed}=1$ iff $\texttt{v\_mean} \geq 0.05 \land \texttt{v\_max} \leq 1.0$ \\

RQ3 &
Safe stopping distance &
$\texttt{RQ3\_SafeDistance}=1$ iff $\forall i, |d_i - 0.80| \leq 0.30$ \\

RQ4 &
Stable Perception &
$\texttt{RQ4\_Perception}=1$ iff $\texttt{track\_err\_rms} \leq 150$ \\

\bottomrule
\end{tabular}
\end{table*}

\subsection{Simulation execution}
The co-simulation campaign was executed on an HP EliteBook 840 G10 workstation equipped with a 13th Gen Intel Core i7-1370P processor and 64 GB of RAM, running Ubuntu 22.04.5 LTS. The models and control logic were executed using MATLAB/Simulink (2024a), interfaced via ROS with Gazebo. The Gazebo simulation and TurtleBot3 physical kinematics are hosted within a Virtual Machine.

The configuration setup is executed in co-simulation for 108 runs. Some runs were removed because of errors and missing values required for the influence analysis, and 104 runs remained for influence refinement. 
%, and produces time-stamped traces and logged signals. 
As we defined in the methodology, the co-simulation must log signals required for SRP computation and requirement assessment, such as state estimates, control commands, perception outputs, mode changes, and timing information. The analysis will evaluate the influence models using \texttt{TravelTime} as the output SRP for $I_1$, \texttt{DistanceToSign} as the output SRP for $I_2$, \texttt{RobotMovement} as the output SRP for $I_3$, and \texttt{QualityPerception} as the output SRP for $I_4$.


% The SPRs \texttt{CompletionFlag} and \texttt{CompletionTime} are direcly related to the satisfaction of the requirement RQ1:
% \begin{equation*}
%     \texttt{CompletionFlag} = true \land \texttt{CompletionTime} \leq 60
% \end{equation*}

% The SRPs \texttt{TrackingStability} and \texttt{SignDetectionRate} are indirectly related to the satisfaction of RQ1. They form intermediate influences.

\subsection{Comparison, refinement, and compensation}

%The campaign explores 108 configurations, ranging the configurations of the selected participants. Each configuration is executed n times, with randomized run order. For each run, we log signals from the simulink blocks, compute SRPs, and evaluate requirement satisfaction. We discard invalid runs caused by miscommunication between the simulink and gazebo.

%Across n runs, the workflow revealed that.. 
%For influence $I_2$, we estimate a linear regression model from $[w_{gain},SignDetectionRate]$ to \texttt{TrackingStability}. The fitted model achieved R2 = , and RMSE, under .. This results show that simulation can refine a partial influence relation into a quantitaively analyzabe function.


The structured analysis shows important outcomes for the initially defined influences. First, the relation $I_1 = (blobsize, luminosity_{level}) \rightarrow SignDetectRate$ is strongly supported by the data. The fitted interaction model achieves $R^2=0.756$ with $RMSE=0.185$, showing that the sign-detection response is can be explained by the selected participants. The most impactful participant is luminosity: low luminosity causes a decrease in detection rate, while increasing the blob-size threshold provides a less impactful compensation. The fitted function relating is given by:


\begin{equation}
\widehat{\texttt{SignDetectRate}}
= 0.851 + 0.000707\,\texttt{blob\_size} 
- 0.581603\,\texttt{L\_low} 
- 0.000491\,\texttt{blob\_size}\,\texttt{L\_low},
\end{equation}

where $L_{\mathrm{low}}$ is a binary indicator equal to 1 under low luminosity and 0 under high luminosity.

This function also makes explicit that increasing $blobsize$ has a greater effect in the detection rate under high luminosity than under low luminosity.

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{images/interaction_signdetection.png}
\caption{Influence of Blobsize threshold and illumination level on Sign Detection Rate.}
\label{fig:i1}
\end{figure}

The relation $I_2 = (w_{gain}, SignDetectRate) \rightarrow TrackingStability$ is moderately supported by the data. The fitted model achieves $R^2=0.530$ and $RMSE=0.342$, indicating that the selected participants explain part of the observed stability variation, although not all of it. The fitted function relating those participants is defined as:

\begin{equation}
    \widehat{TrackingStable}=-0.223+0.512299\,w_{gain}+1.059707\,SignDetectRate-0.322003\,w_{gain}\,SignDetectRate
\end{equation}

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{images/i2.png}
\caption{Influence of wGain and sign detection on Tracking Stability.}
\label{fig:i1}
\end{figure}


The relation $I_3 = (v_{nominal}, friction_{surface}) \rightarrow TravelSpeed$ resulted to be weekly supported by the simulation campaign. The fitted model results in only $R^2=0.032$ with $RMSE=0.146$, which indicates that the participants alone do not explain the realized mean travel speed. A low value of $R^2$ shows that this influence should not yet be treated as a reliable quantitative refinement. This is still useful information, indicating the need of further simulation campaigns, exploration of possible participants in this influence.

\begin{equation}
    \widehat{TravelSpeedMean}=0.086+0.330946\,v_{nominal}+0.041266\,F_{low}-0.057544\,v_{nominal}\,F_{low}
\end{equation}

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{images/i3.png}
\caption{Influence of friction and $v_{nominal}$ on Travel Speed Mean.}
\label{fig:i1}
\end{figure}

\begin{table*}[h!]
\centering
\caption{Learned influence functions and model quality. $L_{low}=1$ represents $luminosity_{level}=low$, otherwise 0. $F_{low}=1$ when $friction_{surface}=low$, otherwise 0.}
\label{tab:learned-influences}
\begin{tabular}{p{0.7cm} p{13.0cm} c c}
\toprule
Infl. & Learned function & $R^2$ & RMSE \\
\midrule
$I_1$ &
$\widehat{SignDetectRate}=0.851+0.000707\,blobsize-0.581603\,L_{low}-0.000491\,blobsize\,L_{low}$ &
0.756 & 0.185 \\
$I_2$ &
$\widehat{TrackingStable}=-0.223+0.512299\,w_{gain}+1.059707\,SignDetectRate-0.322003\,w_{gain}\,SignDetectRate$ &
0.530 & 0.342 \\
$I_3$ &
$\widehat{TravelSpeedMean}=0.086+0.330946\,v_{nominal}+0.041266\,F_{low}-0.057544\,v_{nominal}\,F_{low}$ &
0.032 & 0.146 \\
\bottomrule
\end{tabular}
\end{table*}
% \begin{itemize}
%     \item Perception: subscribes to the camera topic, performs image processing, and publishes sign signals such as \texttt{detected}, \texttt{$blob_{size}$}, and \texttt{$blob_{X}$}.
%     \item Decision: takes as input sign signals, executes tracking logic including scan, track and stop, and outputs a motion command \texttt{v,w,stop}.
%     \item Motion: converts motion commands to wheel/drive commands and applies constraints for generating actuation.
% \end{itemize}


